Network architecture of energy landscapes in mesoscopic quantum systems

Mesoscopic quantum systems exhibit complex many-body quantum phenomena, where interactions between spins and charges give rise to collective modes and topological states. Even simple, non-interacting theories display a rich landscape of energy states --- distinct many-particle configurations connected by spin- and energy-dependent transition rates. The collective energy landscape is difficult to characterize or predict, especially in regimes of frustration where many-body effects create a multiply degenerate landscape. Here we use network science to characterize the complex interconnection patterns of these energy-state transitions. Using an experimentally verified computational model of electronic transport through quantum antidots, we construct networks where nodes represent accessible energy states and edges represent allowed transitions. We then explore how physical changes in currents and voltages are reflected in the network topology. We find that the networks exhibit Rentian scaling, which is characteristic of efficient transportation systems in computer circuitry, neural circuitry, and human mobility, and can be used to measure the interconnection complexity of a network. Remarkably, networks corresponding to points of frustration in quantum transport (due, for example, to spin-blockade effects) exhibit an enhanced topological complexity relative to networks not experiencing frustration. Our results demonstrate that network characterizations of the abstract topological structure of energy landscapes can capture salient properties of quantum transport. More broadly, our approach motivates future efforts to use network science in understanding the dynamics and control of complex quantum systems.

==> LCB_macros.tex <==
% List of definitions and other useful macros from LCB thesis:

% Environment for system of equations array, with left curly brace:
\newenvironment{sistema}{%
    \left\lbrace\begin{array}{@{}l@{}}}
{\end{array}\right.}

\newcommand\figref[1]{Fig.~\ref{#1}}
\newcommand\figvref[1]{Fig.~\ref{#1}\vpageref{#1}}
\newcommand\figsref[1]{Figs.~\ref{#1}}
\newcommand\eqnref[1]{Eq.~\eqref{#1}}
\newcommand\eqnvref[1]{Eq.~\eqref{#1}\vpageref{#1}}
\newcommand\eqnsref[1]{Eqs.~\eqref{#1}}
\newcommand\secref[1]{\S\ref{#1}}
\newcommand\chapref[1]{Chapter~\ref{#1}}
\newcommand\chapsref[1]{Chapters~\ref{#1}}
\newcommand\appref[1]{Appendix~\ref{#1}}
\newcommand\refref[1]{Ref.~\cite{#1}}
\providecommand{\abs}[1]{\lvert#1\rvert}%
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}%
\providecommand{\smallERsum}[1]{{\sideset{}{^\varepsilon}{\textstyle\sum}\limits_#1}}%
\providecommand{\ERsum}[1]{{\sideset{}{^\varepsilon}{\sum}\limits_#1}}%
\providecommand{\smallsum}[2]{\textstyle\sum\limits_{#1}^{#2}}
\providecommand{\bra}[1]{\langle#1\rvert}
\providecommand{\ket}[1]{\lvert#1\rangle}
\DeclareMathOperator{\Tr}{Tr}%
\DeclareMathOperator{\sign}{sgn}%
\DeclareMathOperator{\var}{var}%
\DeclareMathOperator{\stdev}{stdev}%
\DeclareMathOperator{\mean}{mean}%

\def\omegac{\omega_\mathrm{C}}
\def\ellB{\ell_\mathrm{B}}
\def\Ef{E_\mathrm{F}}
\def\Ez{E_\mathrm{Z}}
\def\Ec{E_\mathrm{C}}
\def\Eex{E_\mathrm{ex}}
\def\Ead{E_\mathrm{AD}}
\def\Rad{R_\mathrm{AD}}
\def\nuAD{\nu_\mathrm{AD}}
\def\nuB{\nu_\mathrm{B}}
\def\dEsp{\Delta E_\mathrm{SP}}
\def\HSP{\hat{h}}
\def\bx{\mathbf{x}}
\def\esp{\varepsilon^\mathrm{SP}}
\def\ehf{\varepsilon^\mathrm{HF}}
\def\etaC{\eta_\mathrm{C}}
\def\Nup{N_\uparrow}
\def\Ndn{N_\downarrow}
\def\Nhup{N^\mathrm{h}_{\uparrow}}
\def\Nhdn{N^\mathrm{h}_{\downarrow}}
\def\Nh{N_\mathrm{h}}
\def\neupvec{\mathbf{n}^\mathrm{e}_{\uparrow}}
\def\nednvec{\mathbf{n}^\mathrm{e}_{\uparrow}}
\def\nhupvec{\mathbf{n}^\mathrm{h}_{\uparrow}}
\def\nhdnvec{\mathbf{n}^\mathrm{h}_{\downarrow}}
\def\nupvec{\mathbf{n}_\uparrow}
\def\ndnvec{\mathbf{n}_\downarrow}
\def\spinup{spin\nobreakdash-$\uparrow$}
\def\spindn{spin\nobreakdash-$\downarrow$}
\def\onetothree{1$\leftrightarrow$3}
\def\twotofour{2$\leftrightarrow$4}
\def\onetoone{1$\leftrightarrow$1}
\def\twototwo{2$\leftrightarrow$2}
\def\rvec{\mathbf{r}}
\def\dsD{\overleftrightarrow{\mathbf{D}}}
\def\ainvec{\mathbf{a}^\mathrm{in}}
\def\aoutvec{\mathbf{a}^\mathrm{out}}
\def\finj{f_\mathrm{Inj}}
\def\fdet{f_\mathrm{Det}}
\def\fdettwo{f_\mathrm{Det2}}
\def\Gneq{G_\mathrm{Neq}}
\def\Gdrain{G_\mathrm{Drain}}
\def\Gdet{G_\mathrm{Det}}
\def\Gtot{G_\mathrm{Tot}}
\def\Gaup{G_{2\mathrm{T}\alpha}}
\def\Gap{G_{2\mathrm{T}\alpha^\prime}}
\def\G2t{G_\mathrm{2T}}
\def\Gup{G_\uparrow}
\def\Gdn{G_\downarrow}
\def\Vug{V_\mathrm{UG}}
\def\Vlg{V_\mathrm{LG}}
\def\Vad{V_\mathrm{AD}}
\def\Vex{V_\mathrm{EX}}
\def\Vsd{V_\mathrm{SD}}
\def\Vds{V_\mathrm{DS}}
\def\ils{\ell_\mathrm{SF}^{-1}}
\def\ilo{\ell_\mathrm{LL}^{-1}}
\def\lsf{\ell_\mathrm{SF}}
\def\lLL{\ell_\mathrm{LL}}
\def\aout{a^\mathrm{out}}
\def\nbd{\nobreakdash\textendash}
\def\GammaD{\Gamma^\mathrm{D}}
\def\GammaS{\Gamma^\mathrm{S}}
\def\gDup{\Gamma_{\mathrm{D}\uparrow}}
\def\gSup{\Gamma_{\mathrm{S}\uparrow}}
\def\gDdn{\Gamma_{\mathrm{D}\downarrow}}
\def\gSdn{\Gamma_{\mathrm{S}\downarrow}}
\def\muup{\mu_\uparrow}
\def\mudn{\mu_\downarrow}
\def\musf{\mu_\mathrm{SF}}
\def\eSOI{\varepsilon_\mathrm{SOI}}
\def\eHF{\varepsilon_\mathrm{HF}}
\def\Etherm{E_\mathrm{Therm}}
\def\mueV{\micro\electronvolt}
\def\dmuup{\Delta\mu_\uparrow}
\def\Npone{N\!+\!1}
\def\Nmone{N\!-\!1}
\def\Cs{C_\mathrm{S}}
\def\Cd{C_\mathrm{D}}
\def\Cg{C_\mathrm{G}}
\def\Cr{C_\mathrm{R}}
\def\Vs{V_\mathrm{S}}
\def\Vd{V_\mathrm{D}}
\def\Vg{V_\mathrm{G}}
\def\nG{n_\mathrm{G}}
\def\muD{\mu_\mathrm{D}}
\def\muS{\mu_\mathrm{S}}
\def\mudot{\mu_\mathrm{dot}}
\def\alphaG{\alpha_\mathrm{G}}
\def\alphaD{\alpha_\mathrm{D}}
\def\ksr{{k\sigma r}}
\def\kls{{k\ell\sigma}}
\def\ls{{\ell\sigma}}
\def\lps{{\ell^\prime\sigma}}
\def\sptos{{s^\prime\rightarrow s}}
\def\kptok{{\chi^\prime\rightarrow \chi}}
\def\llps{{\ell\ell^\prime\sigma}}
\def\sp{{s^\prime}}
\def\gSrssp{\gamma^\Sigma_{r,s\sp}}
\def\mussp{\mu_{s\sp}}
\def\dEs{\Delta E_S}
\def\dEt{\Delta E_{T_0}}
\def\Szz{S_{z0}}
\def\El{\varepsilon_L}
\def\Es{\varepsilon_S}
\def\Rs{R_\mathrm{S}}
\def\Rd{R_\mathrm{D}}
\def\nL{n_\mathrm{L}}
\def\nS{n_\mathrm{S}}
\def\Btot{B_\mathrm{Tot}}
\def\Bperp{B_\perp}

